Broadband, millimeter-wave anti-reflective structures on sapphire ablated with femto-second laser

We designed, fabricated, and measured anti-reflection coating (ARC) on sapphire that has 116% fractional bandwidth and transmission of at least 97% in the millimeter wave band. The ARC was based on patterning pyramid-like sub-wavelength structures (SWS) using ablation with a 15 W femto-second laser operating at 1030 nm. One side of each of two discs was fabricated with SWS that had a pitch of 0.54 mm and height of 2 mm. The average ablation volume removal rate was 1.6 mm$^{3}$/min. Measurements of the two-disc sandwich show transmission higher than 97% between 43 and 161 GHz. We characterize instrumental polarization (IP) arising from differential transmission due to asymmetric SWS. We find that with proper alignment of the two disc sandwich RMS IP across the band is predicted to be 0.07% at normal incidence, and less than 0.6% at incidence angles up to 20 degrees. These results indicate that laser ablation of SWS on sapphire and on other hard materials such as alumina is an effective way to fabricate broad-band ARC.

==> Development_of_SWS_on_sapphire_using_laser_ablation_AIP_v7(last)/sec_conclusion.tex <==

SWS have advantages as ARC because they obviate the need for multiple materials and glues with precisely tuned indices of refraction, and because the index gradient produced can be smoother and tailored to specific applications. SWS are superior for cryogenic applications, because there is no need to match materials with different coefficients of thermal expansion.  Fabricating SWS on alumina and sapphire -- materials that have favorable optical properties in the millimeter and sub-millimeter wave band -- using standard machining approaches has been challenging because both materials are among the hardest available. They rank 9/10 on the relative hardness Mohs scale, and sapphire (alumina) has a value of 2500 (2000) HV on the Vickers hardness scale. In this paper we have extended our development of laser ablation as a tool to fabricate SWS for the millimeter and sub-millimeter band. We demonstrated structures on sapphire with aspect ratio $a = 3.7$. The newly fabricated SWS give a working bandwidth of 130\% with transmission above 90\% centered on 97~GHz, and of 116\% with transmission of at least 97\% centered on 102~GHz, arguably the largest bandwidths yet demonstrated in this wavelength range.

Using shorter pulse duration higher power laser and a more efficient fabrication process we have accelerated the AVRR for sapphire by a factor of 18 to 1.6 mm$^{3}$/min. Further acceleration is achievable with increase in laser power~\cite{Neuenschwander,boerner2019} and improvements in fabrication efficiency.

Although the native material was  non-birefringent we found shape asymmetries in the fabricated SWS. The origin of the asymmetries is yet to be understood. However, calculations show that proper relative alignment of samples reduces the magnitude of induced instrumental polarization due to differential reflection by a factor of 35 to 0.07\% at normal incidence, and to less than 0.6\% for incidence angles up to 20 degrees. Measurements at normal incidence are consistent with these predictions as they show the expected reduction in instrumental polarization, but are currently limited to an upper limit of 1\%.

These results and newer ones showing even higher ablation rates~\cite{wen_inprep} indicate that laser ablation of SWS on sapphire and on other hard materials such as alumina is an effective way to fabricate broad-band ARC; the technique has particularly strong advantages in the case of cryogenic applications. 

==> Development_of_SWS_on_sapphire_using_laser_ablation_AIP_v7(last)/sec_design.tex <==

%\comblue{I think the material in the next two paragraphs is needed, although it could go to the introduction, if so preferred. }


LiteBIRD's LFT, one of three telescopes aboard the spacecraft~\cite{sugai}, will operate over a frequency range between 34 and 161~GHz. The focal plane will have about 1200 bolometric detectors tuned to nine broad-band, $\sim$25\% fractional bandwidth frequency bands.  A single HWP placed at the entrance aperture of the LFT will modulate the polarization of sky signals across the entire bandwidth. Thus, the goal is to demonstrate SWS ARC with 130\% fractional bandwidth centered on 97~GHz.

Klopfenstein (Ref.~\onlinecite{Klopfenstein}) derived a prescription for impedance matching between free space and a sample of index $n$. The prescription gives an optimal index of refraction profile and depends on a parameter $\Gamma_{m}$ that controls the trade-off between the lowest frequency of the passband and transmission ripple in-band~\cite{Grann}. All values of $\Gamma_{m}$ between 0.01 and 0.1 give average band transmission between 98\% and 99\%, and we chose $\Gamma_{m} =0.055$ as a fiducial value. With this value average transmission is near 99\%. There are several approaches to transforming the index profile to a physical shape but there is no single closed-form solution~\cite{Grann, Chen:95}. 
%We use an empirical approach
We employ an empirical design approach: we construct physical shapes and use effective medium theory (EMT)~\cite{EMT} and rigorous coupled-wave analysis (RCWA)~\cite{1457488,Moharam} to calculate the resulting index profile. We choose the physical shape that most closely reproduces the desired Klopfenstein index profile. RCWA calculations were carried out using DiffractMOD~\cite{diffractmod}.

%augmented by calculations using effective medium theory (EMT)~\cite{EMT} and rigorous coupled-wave analysis (RCWA)~\cite{1457488,Moharam}. RCWA calculations were carried out using DiffractMOD~\cite{diffractmod}.

We model the SWS as a grid of identical pyramids, see Figure~\ref{fig:Shape_parameters}.  We search for a pyramid shape that closely matches the Klopfenstein index profile by constructing a shape function that gives the width of the pyramid as a function of distance $z$ from the substrate material
\begin{equation}
    w(z) = w_0 + \left\{(p-b)-w_0\right\}\left\{1-(z/h)^{\alpha}\right\},
%    \label{width}
\label{eq:alpha}
\end{equation}
where the parameters are defined in Figure~\ref{fig:Shape_parameters}. 
A value of $\alpha=1$ gives linear slopes; smaller (larger) values give concave (convex) slopes. We considered several values for $\alpha$, but in all cases used $p = 0.54$~mm and $h=2.0$ mm, giving $a=3.7$. The pitch $p$ is set by requiring that at normal incidence the smallest value of the highest pass-band frequency be $\nu_{high} = c/p \, n_{s} = 180$~GHz. Thus $p=\lambda_{high}/n_{s}=0.54$~mm, where $n_{s} = 3.06$ is the index of c-cut sapphire. Smaller value of $p$ implies shorter $\lambda_{high}$, higher $\nu_{high}$, and thus larger bandwidth. In Section~\ref{sec:non_normal} we discuss non-normal incidence. Guidance for the minimum required $h$ is obtained by considering the lowest pass-band frequency and applying the standard criterion for maximum transmission with a single ARC layer that has a uniform index $n_{l}$. In that case $n_{l}=\sqrt{n_{s}}$, and the thickness of the layer should be $t=\lambda_{0}/4n_{l}$, where $\lambda_{0}$ is the vacuum wavelength. 
%\comred{Since a Klopfenstein taper degenerates to a usual quarter-wavelength design if the change of impedance along the height adiabatically approaches 0, the height driven by the quarter-wavelength design is adopted here as a convenient reference.} \comblue{(SH: I don't understand what this says.)} 
For the pyramids we found empirically that $h$ should satisfy $h \gtrsim \lambda_{0}/3n_{l} = 1.9$~mm, where $\lambda_0=8.8~$mm.
%\comgreen{\cite{kamizuka}}. \comblue{The addition of this reference is out of place. the sentence says that "*we* found empirically ...", and then we give a reference to someone else's publication... Also, why has this been added? I looked at the paper and I don't quite see the connection to this sentence. } 
We required $h \geqq 2.0$~mm.
%\comcyan{Correspondingly, the aspect ratio, height/pitch$\equiv a$, is $a\geqq3.7$.}
The choice of $w_0$ was determined iteratively by trying several values. We determined that $w_0=0.1$~mm is the largest value that would still give an effective index that matches the Klopfenstein profile. Larger values produce a mismatch of the indices near $n=1$. We assumed that the deep laser ablated grooves will give $b=0$ making $p=p'$ (see Figure~\ref{fig:Shape_parameters}).
%\comgreen{\cite{tomo_ISSTT}}. \comblue{1. See earlier comment regarding citation 27; 2. Even if the citation is included properly, does the ISST paper *prove* that $p=p'$?}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{Figure_file/parameter_settings.jpg}
    \caption{Geometrical parameters of pyramidal-shaped SWS. The shape of the pyramids (right panel) is controlled by a parameter $\alpha$ defined by Equation~\ref{eq:alpha}. Other parameters are the tip width $w_0$, the period $p$, the width at the bottom of the pyramid $p^\prime$, the groove width $b$, and the height $h$.
    \label{fig:Shape_parameters} }
\end{figure}
We used second-order EMT to calculate the effective index of refraction as a function of $\alpha$, and RCWA to calculate the expected transmission as a function of frequency; see Figure~\ref{fig:RCWA_profile_trans}. A convex pyramid shape with $\alpha = 1.5$ gives an index profile that closely matches the Klopfenstein profile with the fiducial $\Gamma_{m}$. The average band transmissions for $\alpha = 1.0, \, 1.5$ and 2 are 97.7\%, 98.4\%, and 98.3\%, respectively; see Figure~\ref{fig:RCWA_profile_trans}. 
The sharp reflection features apparent in the Figure above 180~GHz are due to the onset of diffraction.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{Figure_file/alpha_dependence_20200507_ver4.jpg}
    \caption{Top: EMT-calculated index profiles for four values of $\alpha$ (colored lines, Equation~\ref{eq:alpha}), and the Klopfenstein index profile with $\Gamma_{m} = 0.055$ (black). The other physical parameters used to calculate the index profiles are $h=2.0$ mm, $p = 0.54$~mm, $w_0=0.1$~mm, and $b=0$. Bottom: calculated transmittance as a function of frequency for SWS designs with the parameters given in the upper panel. Sharp reflection features above 180~GHz are due to the onset of diffraction. 
    \label{fig:RCWA_profile_trans} }
\end{figure}




==> Development_of_SWS_on_sapphire_using_laser_ablation_AIP_v7(last)/sec_discussion.tex <==




%\sout{The two-dimensional rectangular-like nature of the $z$-axis projection of the SWS is a potential source of polarimetric systematic effects.}
Systematic asymmetry in fabrication along the two orthogonal axes, due to laser beam polarization or birefringent material properties (if such is used), leads to different effective indices of refraction along the two axes. Differential index causes differential transmission, which is a source of instrumental polarization (IP), the conversion of unpolarized to polarized light by the optical element. Even when the structures are two-dimensional symmetric there is differential reflection at non-normal incidence, as there would with any ARC scheme; differences in transmission between S and P polarization states of the incident light lead to IP. 

To quantify the IP induced by normal incidence differential transmission we use the figure of merit~\cite{radio_astronomy,karl} 
\begin{align}
    {\rm IP}(\nu) & =  \frac{ T_x(\nu) - T_y(\nu)  }{T_x(\nu) + T_y(\nu)} 
\label{eq:asymmetry_nophi} \\
    & =  \frac{ T(\phi=0^{\circ}, \nu) - T(\phi=90^{\circ}, \nu)  }{T(\phi=0^{\circ}, \nu) + T(\phi=90^{\circ}, \nu)} ,
\label{eq:asymmetry_phi1}
\end{align}
where we have introduced in the last expression the relative rotation angle $\phi$ between the $x$ orientation of the sample and the direction along which transmission is probed. IP vanishes for normal incidence light when the substrate and ARC are $z$-projected isotropic. At normal incidence  Equations~\ref{eq:asymmetry_nophi} and~\ref{eq:asymmetry_phi1} could have been written equivalently in terms of $T_{s} \equiv T(\phi=0^{o}) $ and $T_{p} \equiv T(\phi=90^{o})$, the transmissions for S and P polarization states.
 
At non-normal incidence and in the presence of $x$-$y$ ARC asymmetry $T_{s}$ and $T_{p}$ depend on both the angle of incidence $\theta_{i}$ and on the azimuthal angle $\phi$ of the plane of incidence, measured relative to $x$. We now have  
 \begin{equation}
    {\rm IP}(\phi,\theta_i,\nu) = \frac{ T_s(\phi,\theta_i,\nu) - T_p(\phi,\theta_i,\nu)  }{T_s(\phi,\theta_i,\nu) + T_p(\phi,\theta_i,\nu)}
\label{eq:asymmetry_phi2}
\end{equation} 
see Figure~\ref{fig:inc_pol_iamge}.
%\comblue{the equation uses $\theta_{i}$, the figure uses $\theta$. Please make uniform}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figure_file/pol_image.jpg}
    \caption{A diagram showing the variables of Equation~\ref{eq:asymmetry_phi2}. The transmissions $T_{p}$ and $T_{s}$ are for light polarized parallel and perpendicular to the plane of incidence, respectively.}
    \label{fig:inc_pol_iamge}
\end{figure}

In the following two Sections we quantify systematic effects due to asymmetry in the fabricated SWS at normal incidence (Section~\ref{sec:asymmetry}) and due to non-normal incidence (Section~\ref{sec:non_normal}), and discuss the level of mitigation provided by appropriately stacking the two-disc sandwich. We refer to `parallel' and `perpendicular' configurations, in which the two plates are stacked with their $x$ axes parallel, or with $x$ of one perpendicular to $x$ of the other, respectively. In the perpendicular configuration the quantities $T_{x}$ and $T_{y}$ refer to transmission measurements relative to the $x$ axis of the source-side sample of the stack, which was Sample1. 

\subsection{Asymmetry of SWS at normal incidence}
\label{sec:asymmetry}

Figure~\ref{fig:IP} shows IP inferred from the measured data (Figure~\ref{fig:pharos_trans}) for the individual samples and when stacked in the parallel and perpendicular configurations. It also shows the calculated response (using RCWA) using the average parameters for the $x$ and $y$ orientations in Table~\ref{tab:geometrical_measurement_parameters_table}. We find values of IP reaching 10\% at frequencies below 100~GHz for the individual samples, and below 50~GHz for the parallel stacking. For the entire bandwidth the RMS IP is 2.5\%. 
At frequencies higher than 50~GHz, 
IP in the parallel stacking configuration is smaller than in the individual samples because of higher transmission and because of some averaging of the two somewhat different asymmetries. 

However, when the plates are stacked in the perpendicular configuration we find lower IP across the band as shown in the bottom panel of Figure~\ref{fig:IP}. 
The data and the RCWA prediction are consistent within measurement errors, which take into account residual standing waves (see Section~\ref{sec:transmission}).
If the errors are assumed to be statistical, we find an upper limit of 1\% on the RMS across the band. 
The RMS IP calculated based on RCWA is 0.07\%, a value that is nearly 35 times smaller than in the parallel configuration, and is below our  measurement limits.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figure_file/20191107_pharos89_measurement_IP_v4.jpg}
    \caption{
    Instrumental polarization due to differential transmission IP for each of the samples and when stacked with $x$ axes parallel and perpendicular (blue data points), and RCWA predictions for IP (solid, red) based on the average measured values (Table~\ref{tab:geometrical_measurement_parameters_table}). For perpendicular stacking, calculated RMS IP for the bandwidth is 0.07\%. The vertical dashed line shows the 90~GHz frequency for which we made measurements as a function of stack rotation angle; see Figure~\ref{fig:rotation}.
    \label{fig:IP} }
\end{figure}{}

Figure \ref{fig:rotation} gives data and RCWA predictions for normal incidence transmittance as a function of stacked sample rotation angle $\phi$ for the two configurations at 90~GHz. Concentrating on the parallel configuration first, the effective differential index in $x$ and $y$ is an effective stack birefringence that causes 8.6\% modulation as a function of $\phi$ with $\pi/2$ periodicity only with fully polarized incident light. 
That is, the measurements, which were conducted with fully polarized light, give
 \begin{equation}
    0.086 = \frac{ \bar{T}(\phi=0^{\circ}) - \bar{T}(\phi=45^{\circ})  }{\bar{T}(\phi=0^{\circ}) + \bar{T}(\phi=45^{\circ})}, 
\label{eq:asymmetry_phi}
\end{equation} 
with $\theta_{i} = 0^{o}$, $\nu=90$~GHz, and $\bar{T}$ indicates that we average all $T$ values at the $\phi$ indicated and with $\pi/2$ periodicity. If the experiment and simulation were conducted with partially polarized or  unpolarized light, this $\pi/2$-periodic modulation would have diminished or vanished, respectively. For the HWP, SWS using a-cut sapphire, $\pi/2$ effect also could be vanished with unpolarized light. For Given measurement errors in this band of frequencies, the $\pi/2$-periodic modulation of 0.086 has an uncertainty of 0.014. 

The IP signal due to differential transmission has $\pi$ periodicity. Given the $1\sigma = 1.4\%$ measurement uncertainty the data only give a $2\sigma$ upper limit of IP $<2.8\%$, when calculated using Equation~\ref{eq:asymmetry_phi1}. 
This value is consistent with the IP value at 90~GHz in the third panel of Figure~\ref{fig:IP}, $3 \pm 1.4\%$. This level would persist if the measurement was done with unpolarized light. 
In the perpendicular configuration both the $\pi/2$ and $\pi$-periodic modulation amplitudes, calculated using Equations~\ref{eq:asymmetry_phi} and \ref{eq:asymmetry_phi1}, are consistent with zero within measurement errors. 

The transmission data as a function of $\phi$, such as presented in Figure~\ref{fig:rotation}, reveal that measurements at only two orientations $x \, (\phi=0)$ and $y\, (\phi=90^{o})$ as shown in Figure~\ref{fig:IP} and IP calculated using Equation~\ref{eq:asymmetry_nophi} combine information from distinct physical effects. The effects correspond to, and can be quantified with higher accuracy using decomposition to Fourier harmonics\cite{Hanany:05,kkomatsu}. We fit the data of Figure~\ref{fig:rotation} to the model  
\begin{align}
    &T(\phi,\nu=90\mbox{~GHz})  =  & \nonumber \\
    &    a_0 + a_2\cos{(2\phi + 2C_2)} + a_4\cos{(4\phi + 4C_4),} &
    \label{eq:fourier}
\end{align}
and constrain the amplitudes and phases. We find 
IP$=a_2/a_0=1.6 \pm 0.2\%$ and $0.21\pm 0.22\%$, in the parallel and perpendicular configurations, respectively; and $a_4/a_0 = 7.9\pm 0.2\%$ and $0.07\pm 0.22\%$, respectively, for the effect of stack birefringence. The data in the perpendicular configuration is consistent with zero we thus quote an upper limit of 0.5\% on the values of $a_2/a_0$ and $a_4/a_0$. 
We find that (1) 
the $\pi$ and $\pi/2$ periodic modulations quantified through $a_2/a_0$ and $a_4/a_0$ are more tightly constrained compared to using Equations~\ref{eq:asymmetry_phi1} and~\ref{eq:asymmetry_phi}; (2) the modulation amplitude constraints calculated using the two techniques are consistent; (3) there is a significant detection of IP, that is, $\pi$ periodic modulation, in the parallel case but not in the perpendicular case; and (4) the relatively large 7.9\% $\pi/2$ periodic modulation measured in the parallel case is not detectable in the perpendicular case. 

With the structures as fabricated, perpendicular stacking is predicted to constrain IP to below 0.5\% at 90~GHz, a value that is limited by measurement uncertainty, not by inherent asymmetry. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figure_file/pharos89_rotation_20200703.jpg}
    \caption{Stacked sample transmittance at 90~GHz (blue points) as a function of stack rotation angle $\phi$ for the parallel (top two panels) and perpendicular (bottom two panels) configurations, and RCWA predictions based on the measured parameters in Table~\ref{tab:geometrical_measurement_parameters_table} (red solid). The lower panel in each pair has a limited range for the ordinate values. Shaded regions indicate the 2\% systematic uncertainty we assign to each data point in this frequency. The statistical uncertainty per data point is 0.2\%.
    \label{fig:rotation} }
\end{figure}{}


\subsection{Non-normal incident light}
\label{sec:non_normal} 


Optical systems are designed to admit rays over a range of incidence planes and angles and thus  
calculations of systematic effects arising from ARC SWS asymmetry should take account of the entire range of incidence planes and angles. Including the full range amounts to averaging that gives smaller systematic effects compared to using a single incidence plane and the extreme incidence angle. In the discussion below we analyze the effects of non-normal incidence angles {\it without} any such averaging, and therefore the quantitative values should be understood as upper limits. The analysis relies solely on RCWA calculations of the perpendicular configuration; we have already established that this configuration has smaller level of systematic effects. 

The upper panel of Figure \ref{fig:pharos89_inc} shows calculated IP$(\phi=0)$ as a function of frequency for normal incidence and for the 5, 10, 15 and 20 degrees incidence angle.  For normal incidence the calculation is identical to the one shown in the lower panel in Figure~\ref{fig:IP}. The lower panel shows the difference between transmission at normal incidence and at other angles, again for $\phi=0$. For LiteBIRD's maximum planned incidence angle of 15 degrees RMS IP across the band is 0.4\%, an increase of 0.3\% relative to normal incidence. At 20~degrees incidence, RMS IP increases to 0.6\%. For $\phi=90$ degrees, RMS IP values at 15 and 20 degrees incidence are smaller by 0.1\%.  

Onset of diffraction is apparent at lower frequencies with larger incidence angles. For off-normal incidence, the frequency of diffraction onset -- that is, at the lowest order -- is~\cite{Grann,Bruckner:07}
\begin{equation}
    \nu_{d} = \frac{c}{p(n+\sin{\theta_i})},  
\label{eq:diffraction}
\end{equation}
providing qualitative agreement with the RCWA calculation. We do not expect exact quantitative agreement because the RCWA calculation assumes the full average shape information for the two samples, as given in Table~\ref{tab:geometrical_measurement_parameters_table}, whereas Equation~\ref{eq:diffraction} only assumes a periodic array of scattering centers. 


\begin{figure}[h]
    \centering
    \includegraphics[width = 0.48\textwidth]{Figure_file/pharos89_incident_20200612.jpg}
    \caption{RCWA prediction of IP$(\phi=0)$ for various incidence angles (upper panel), and the difference of off-normal incidence spectra with normal incidence spectra (lower panel), all in the case of perpendicular stacking configuration.
    \label{fig:pharos89_inc} }
\end{figure}{}





==> Development_of_SWS_on_sapphire_using_laser_ablation_AIP_v7(last)/sec_fabrication.tex <==


\subsection{Sapphire}
\label{sec:sapphire}

%We procured three samples of c-cut sapphire
%\comred{, cut perpendicular to the c-axis,} from the same ingot
We procured three samples of c-cut sapphire that were cut from the same ingot, each $3.150 \pm 0.002$~mm thick and 100~mm diameter. 
%\comblue{If the referee doesn't know what c-cut is, why would he know what c-axis is? I think we should push back here. This is too trivial to include. A 3 sec google search would tell anyone what c-cut is.} 
We used one sample and the apparatus discussed in Section~\ref{sec:transmission} to measure the index of refraction and loss and obtained $n=3.062 \pm 0.002$ and $\tan{\delta}<1\times10^{-4}$, which is consistent with other data~\cite{Lamb}. In subsequent analysis and simulations we assume that these values are common to all three samples. 
%\comblue{Two topics in progress: 1. significant figures; 2. how to report loss.}

We fabricated the SWS on a circular area of 34.5~mm diameter on one side of each of two samples, to which we refer as Sample 1 and Sample 2. We patterned only one side because LiteBIRD's LFT HWP will be a Pancharatnam multi-stack achromatic HWP~\cite{Pancharatnam1} with SWS only on the outermost surfaces. 
In Section~\ref{sec:transmission} we present transmission measurements of each sample and when they are stacked flat side on flat side. 

Using c-cut, non-birefringent sapphire, simplifies interpretation of the results. At normal incidence, which is the only experimental data we present here, any apparent birefringence is the result of asymmetry in fabrication, not of inherent asymmetry in the material, as would be the case with birefringent a-cut sapphire.




%about laser machine, scan strategy
\subsection{Laser machining}
\label{sec:laser}

The SWS are patterned using a 15~W average power femto-second laser operating at 1030~nm; the laser parameters are given in Table~\ref{tab:laser_specification}. 
The laser beam scans lines in two orthogonal directions to make grooves, and thus produce the pyramids; see Figure~\ref{fig:scan_strategy}. This scan strategy largely follows an approach we used in the past, see for example Young et al. (Ref~\onlinecite{karl}).
The focus position is set at a fixed $z=-0.75$~mm throughout the ablation. The surface of the disk at the beginning of ablation is at $z=0$ and negative values are inside the sample.

\begin{table}[h]
    \centering
    \caption{Laser Specifications}
    \begin{tabular}{c|c}\hline
        \multicolumn{2}{c}{Model:  Pharos, PH1-15W} \\ \hline
         Wavelength & 1030 nm \\
         Repetition rate &  75 kHz\\
         Pulse duration & 290 fs \\
         Pulse energy & 200 $\mu$J \\ %\hline
%\multicolumn{2}{c}{Galvano scanner with f-theta lens (ScanLab)}\\\hline
%         focus distance & 100 mm\\
         Spot diameter ($1/e^2$) & 15.5 $\mu$m \\
    \end{tabular}
    \label{tab:laser_specification} 
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width = 0.4\textwidth]{Figure_file/scan_strategy_20200522.jpg}
    \caption{Sketch of the laser beam scan pattern to fabricate the SWS. Repeated ablation of groups of 53 lines produces grooves. The lines are internally spaced by less than 10 $\mu$m and the groups are separated by at least 72~$\mu$m.  Grooves fabricated in two orthogonal directions leave pyramids, which are the SWS. Layers similar to the one shown in the sketch are repeated 60 times until the desired SWS height is achieved. } 
    \label{fig:scan_strategy}
\end{figure}


\subsection{Characterization of fabricated structures}
\label{sec:charaterization}

The SWS were imaged using confocal imaging. A three-dimensional image of a section of the fabricated region is shown in Figure~\ref{fig:sample_shape}.   Visual inspection indicates that all SWS are physically intact with no breakage nor damaged tips. We measured 160 structures at each of five  locations in each sample, in the center and in four edge regions, and quantified several geometrical parameters as detailed in Figure~\ref{fig:sample_shape} and Table~\ref{tab:geometrical_measurement_parameters_table}. Values given in the Table are averages and standard deviations of the 800 measurements. We established a global cartesian coordinate system that was aligned with the grooves, and for each measured pyramid we defined $xz$ and $yz$ planes that intersected the center of its peak. For both planes (and for each pyramid) we quantified the widths $w_{0x}$ and $w_{0y}$ and two `saddle' heights $d_{x}$ and $d_{y}$, which quantified the depths between pyramids in the $x$ and $y$ directions. The total height $h_{t}$ is given by the depth into trenches in the diagonal direction where the laser beam ablates in both the $x$ and $y$ passes. We best-fit the slopes of the pyramids as imprinted in the $xz$ and $yz$ planes to produce measured $\alpha_{x}$ and $\alpha_{y}$.

\begin{figure}[t]
    \centering
%    \includegraphics[width=0.5\textwidth]{Figure_file/pharos89_shape_ver20200420.jpg}
%    \includegraphics[width=0.5\textwidth]{Figure_file/pharos89_shape_20200512.jpg}
    \includegraphics[width=0.5\textwidth]{Figure_file/pharos89_shape_20200518.jpg}
    \caption{  Left: Confocal microscopy image of a section of the fabricated SWS. The structures are physically intact across the entire sample and the average height is 2~mm. Right: Definition of measurement parameters. Averages of 800 measurements of these parameters are given in Table~\ref{tab:geometrical_measurement_parameters_table}.   
    \label{fig:sample_shape} }
\end{figure}


There is good agreement between the design and fabricated values for the pitch and total height, and there is $x$-$y$ symmetry in the measured pitch. There is good repeatability between the two samples, which were fabricated several days apart. Asymmetry of 5\%-20\% is apparent at the tip of the structures, the saddle heights, and the slope values $\alpha$. This structural asymmetry could have been caused by laser beam polarization, which was not monitored; by the ablation scan strategy, for example the order in which $x$ and $y$ directions were scanned; or by laser beam projection, if the sample was not precisely normal to the beam.
%We will discuss the systematic effects caused by the structure asymmetry in the later section.

It took 10.5~hours to fabricate each sample giving an average volume removal rate (AVRR) of 1.6~mm$^{3}$/min. This rate is 18 times faster than achieved in one of our earlier publications~\cite{tomo_ISSTT}. The higher rate is due to using five times higher averaged power and a more efficient sample scan pattern. Matsumura et al.\ (Ref.~\onlinecite{tomo}) report a higher AVRR of 2.2~mm$^3$/min, but with higher power (25~W) and for SWS with smaller total height of 715~$\mu$m; Schuetz et al.\ (Ref.~\onlinecite{victor}) show that AVRR increases with power and lower structure height. 


Using EMT and the average values given in Table~\ref{tab:geometrical_measurement_parameters_table} we calculated effective index profiles in $x$ and $y$ for each sample; see Figure~\ref{fig:pharos8_9_EMT}. To indicate the variance we included the index profiles for all 800 measured structures as shaded regions. As the values in Table~\ref{tab:geometrical_measurement_parameters_table} indicate, the measured profiles in $x$ match the design profile with $\alpha = 1.5$ better than the measured profiles in $y$.

\begin{table}[t]
    \centering
    \caption{
    Averages of measured geometrical parameters of 800 pyramids measured in five regions of each sample. The parameters are defined in Figure~\ref{fig:sample_shape}. The accuracy of the confocal microscope is 1~$\mu$m in the $xy$ plane and 8~$\mu$m in the $z$ direction.}
    \begin{tabular}{c|c|c|c}
         Parameter     &    Design value & Sample 1 & Sample 2  \\ 
                       &    (mm) & (mm)      & (mm) \\ \hline
        Top width $x$ ($w_{0x}$) & 0.1 & $0.14 \pm 0.01 $ & $0.14 \pm 0.01 $\\
        Top width $y$ ($w_{0y}$) & 0.1 & $0.12 \pm 0.01 $ & $0.12 \pm 0.01 $\\
        Saddle height $x$ ($d_{x}$) & & $1.51 \pm 0.04 $ & $1.52 \pm 0.04 $\\
        Saddle height $y$ ($d_{y}$) & & $1.60 \pm 0.04 $ & $1.59 \pm 0.05 $\\
        Total height ($h_{t}$) & 2.0 & $2.03 \pm 0.04 $ & $2.04 \pm 0.05 $\\
        Pitch $x$ ($p'_{x}$) & 0.54 &  $0.54 \pm 0.01 $ & $0.54 \pm 0.01 $\\
        Pitch $y$ ($p'_{y}$) & 0.54 & $0.54 \pm 0.01 $ & $0.54 \pm 0.01 $\\ \hline 
        $\alpha_x$ $^{\dagger}$ & 1.5& $1.56 \pm 0.06 $ & $1.56 \pm 0.04$\\
        $\alpha_y$ $^{\dagger}$ & 1.5 & $1.22 \pm 0.02 $ & $1.22 \pm 0.02$\\
\hline
\multicolumn{3}{l}{$^{\dagger}$ dimensionless quantity}
    \end{tabular}
    \label{tab:geometrical_measurement_parameters_table}
\end{table}

\begin{figure}[h]
    \centering
%    \includegraphics[width=0.45\textwidth]{Figure_file/pharos89_effn.jpg}
    \includegraphics[width = 0.5\textwidth]{Figure_file/pharos89_effective_index_20200608.jpg}
    \caption{ The effective index of refraction calculated with EMT using the average values of the measured SWS (solid red and green), and with the design values and $\alpha = 1.5$ (solid black). The shaded regions include index profiles for all 800 measured structures.
    \label{fig:pharos8_9_EMT} }
\end{figure}



==> Development_of_SWS_on_sapphire_using_laser_ablation_AIP_v7(last)/sec_intro.tex <==


% 
Sapphire, alumina, and silicon have material properties that make them appealing for use as optical elements in the millimeter and sub-millimeter (MSM) waveband, loosely defined as 30 - 3000 GHz. Compared to plastic-based materials, they have indices of refraction near 3, giving more aberration correction power per unit lens thickness~\cite{Lamb}. They have amongst the lowest absorption loss at room temperature and when cooled to cryogenic temperatures \cite{parshin1995}, and they have thermal conductance higher by factors of hundreds, making them useful for cryogenic applications~\cite{child_1973}. Sapphire has 10\% birefringence making it an ideal half-wave plate (HWP) material for polarimetric applications. 
A number of astrophysical instruments operating in the MSM waveband are using these materials~\cite{Thornton_2016,EBEX2018,SPT-3G,Kaneko2020}. 

The high index of refraction leads to high reflection loss; the average reflectance across 30\% fractional bandwidth of a 1~cm thick slab of non-birefringent sapphire at 150~GHz is 40\%. Reduction of reflection loss is achieved by applying an anti-reflection coating (ARC).  There are two generic approaches for implementing ARC:
%
(i) applying layers of materials with appropriately chosen intermediate indices; and (ii) machining sub-wavelength structures (SWS) on the native optical element material~\cite{Raut2011AntireflectiveCA}. 
%\comblue{(Did you check what are 'resonant structures' in relation to ARC? I don't believe they are related to multi-layer ARC. `Adiabatic tapering' is used, but less often then SWS. I don't think we should use 'metamaterial'. I have no idea what it means; I don't think a definition exists. In summary: what we had was fine. It captures the basic physics.)}
%
%(i) \comred{resonant structures} applying layers of materials with appropriately chosen intermediate indices; and (ii) \comred{adiabatic structures, called as a metamaterial,} machining sub-wavelength structures (SWS) on the native optical element material~\cite{Raut2011AntireflectiveCA}. 
%
An advantage of the SWS approach is that it does not require new materials and glues. This advantage matches well the needs of cryogenic instruments in which differences in coefficients of thermal expansion make the application of multi-layers challenging. Another advantage is that SWS give flexibility in synthesizing any index profile between free space and the substrate material.
%\comred{A single layer coating equivalent ARC using SWS can be realized by an array of the periodic pillar structure or an array of holes. For a broader frequency coverage, prescriptions exist for index profiles that give fractional bandwidths exceeding 100\% with maximal, in some sense optimal, in-band transmission~\cite{Klopfenstein}. 
%This can be realized by fabricating the adiabatic structures.}
Prescriptions exist for index profiles that give fractional bandwidths exceeding 100\% with maximal, in some sense optimal, in-band transmission~\cite{Klopfenstein}. 

Two classes of MSM instruments that require broad-bandwidths and cryogenic optical elements are those mapping the spatial polarization of the cosmic microwave background radiation (CMB)\cite{Johnson_2007,EBEX2018,SPT-3G,Simon2018,Kaneko2020,SO-OverviewGalitzki10.1117/12.2312985,cmb-s4techbookfirsted}, and others measuring the properties of Galactic dust \cite{Dober_blastpol10.1117/12.2054419,blasttngLourie10.1117/12.2314396,nika2pisano2020}. A number of these instruments have used, or plan to use, sapphire as HWP polarization modulator. 
To reduce detector noise the HWP is maintained at cryogenic temperatures, typically near 4~K, and to increase instrument throughput a single HWP operates over a broad range of frequencies, making a single quarter-wave layer of ARC inadequate. Examples of relevant past instruments include Blastpol and EBEX, which had sapphire HWPs with operating bandwidth of 69\% and 109\%, respectively\cite{Dober_blastpol10.1117/12.2054419,EBEX2018}. The bandwidth of the EBEX HWP is the largest reported to date. Ongoing and future experiments include POLARBEAR2, Simons Observatory and LiteBIRD\cite{Kaneko2020,SO-OverviewGalitzki10.1117/12.2312985,sugai}. 

LiteBIRD is a Japanese-led space mission scheduled to be launched late in the next decade~\cite{sugai,YSakurai}. LiteBIRD's low frequency telescope (LFT), designed to operate between 34 and 161~GHz (a fractional bandwidth of 130\%), will have an aperture diameter of 40~cm with a HWP operating at 20~K. Currently no ARC technology on sapphire is available over this broad bandwidth. Implementing SWS ARC for the LiteBIRD HWP has motivated the developments we report in this paper.

Although SWS have advantages as ARC, their implementation on hard materials such as sapphire and alumina present fabrication challenges~\cite{Araujo2016,JAIN20021269,TUERSLEY1994377,machining_difficult}. Broad bandwidths require SWS with aspect ratios $a$ -- defined as height/pitch -- reaching four. 
Diameters of anticipated sapphire and alumina optical elements, which are reaching 80~cm\cite{AliCPTHong10.1093/nsr/nwy019}, require commercially viable machining speed.  
To overcome these challenges we demonstrated a technique to fabricate mm-wave SWS on sapphire, alumina, and silicon using laser micro-fabrication~\cite{tomo,karl,victor,tomo_ISSTT}.  
With laser ablation, which has already been used in the past to ablate these and other materials~\cite{Bonse2002,Ihlemann1995,WANG2004221}, there is no wear and tear of the machining tool. 
Even for materials that can be machined using conventional tools, laser ablation gives finer control of structure shapes, because laser spot diameters can be focused to smaller sizes than other tools. A spot diameter of 16~$\mu$m has been demonstrated at the IR~\cite{HSakurai}; smaller spot diameters are achievable in the UV.
%\comred{The size of the structure by laser machining is limited by the laser spot size, the order of ten micrometer corresponding to THz scale, and the example demonstrations have  been  explored~\cite{HSakurai}. An approach smaller than tens-of-micrometer scale is also developed at typically optical wavelength using a lithography technique, which has a limited applicability to larger structural size, about THz range.}
%\comblue{(SH Comment: I don't think what was written in red was correct. The paper cites 16 micron beam at 1028 nm. (1) this is not `tens-of-micrometer'; (2) at UV we should be able to go down to $\sim \times$10 smaller spot size, certainly less than `tens-of-micrometer'.) } 
Finer control of SWS shapes would give higher transmission over broader bandwidth.
%\comred{Furthermore, a smaller beam spot diameter, a few micrometers using UV laser, can potentially pushes the limit using SWS technology toward the shorter wavelength,}.

Sch\"{u}tz et al.\ and Matsumura et al.\ (Refs.~\onlinecite{victor,tomo}) demonstrated laser-ablated aspect ratios $a =$ 
%\comred{h/p =} 
2.2 and 2.5
%, \comred{where $h$ is the height and $p$ is the pitch},
and heights between 700 and 800~$\mu$m, with sapphire and alumina, respectively. 
%\comblue{(`aspect ratio' is defined above. The referee simply missed it. I added the symbol $a$ above. )}
Young et al.\ (Ref.~\onlinecite{karl}) extended the technique to silicon, showing $a=4$ with height near 700~$\mu$m. To demonstrate applicability to lower frequencies and broader bandwidths, Matsumura et al.\ (Ref.~\onlinecite{tomo_ISSTT}) fabricated structures with $a=5.3$ and total height of 2.1~mm on sapphire. In all of these cases, the volume ablation rate was small, making fabrication of large samples prohibitively expensive; for example, at the rate Matsumura et al.\ (Ref.~\onlinecite{tomo_ISSTT}) quoted for the 2.1~mm tall structures on sapphire it would have taken two months to fabricate a 10~cm diameter sample. 
Further steps in the development of laser micro-fabrication of mm-wave SWS include demonstrating ablation rates that would make commercial fabrication viable with SWS aspect ratios suitable for broad bandwidth applications~\cite{wen_inprep}. In this paper we present progress in the design, fabrication, and characterization of laser-ablated SWS ARC, aiming for 130\% fractional bandwidth ARC centered on 97~GHz with improved fabrication speed. 
In Section~\ref{sec:design}, we present the design of the SWS. Sections~\ref{sec:sample} and~\ref{sec:transmission} give details of the fabrication of two sapphire samples and their transmission properties. We discuss the results and give conclusions in Sections~\ref{sec:discussion} and~\ref{sec:conclusion}.




==> Development_of_SWS_on_sapphire_using_laser_ablation_AIP_v7(last)/sec_measurement.tex <==



We measured the transmittance of the samples at normal incidence between 33 and 190~GHz. The apparatus, a schematic of which is shown in Figure~\ref{fig:plane_wave_setup}, consisted of a source of microwaves, an optical chopper operating at 30 Hz, two parabolic mirrors, a diode detector, and a lock-in amplifier. Between the two mirrors there was an aperture of 30 mm diameter, a sample holder, attenuators to reduce standing waves, and two always identically aligned wire grid polarizers with calculated efficiency exceeding 99\% across the bandwidth. The transmission axis of the polarizers was aligned to within 3~degrees with the $x$ axis of the samples, and the stacked samples were aligned relative to each other to within 0.5 degrees.

To further reduce the effects of standing waves our reported transmittance at each frequency is the average of two transmission measurements taken with the detector positioned at two locations spaced by $\lambda /4$ along the light path. Each transmission measurement is the ratio of power detected with the sample to the power detected without it. 

Measurements of transmission through one of the native samples establish error estimates for subsequent data analysis. We measured transmission using different RF sources at five sub-bands between 33 and 190~GHz; see the top panel of Figure~\ref{fig:flat_measurement}. 
%\comred{The statistical error bars in the transmission measurement are small and not visible in the Figure.} \comblue{check} \comcyan{Yes, it is a high SNR measurement and so the error bar is there ubt it's invisible in this plot.} 
We fit the transmittance to a model with two free parameters, the index of refraction and loss tangent, and find the residuals; see the bottom panel of Figure~\ref{fig:flat_measurement}.  We identify systematic residuals as arising from incomplete cancellation of standing waves and 
%\comred{for all subsequent analyses} \comcyan{this statement looks fine}
quote the RMS of the residual as the error of transmission measurements in each sub-band. They are 6\% (33-50~GHz), 3\% (50-75~GHz), and 2\% (75-190~GHz). 

The errors quoted in Section~\ref{sec:sapphire} for the values of the index of refraction and loss were derived by fitting the transmittance data using statistical errors with magnitude per band as given above and including uncertainty on the measurement of sample thickness. The index and loss errors are dominated by the thickness measurement uncertainty.

\begin{figure}[h]
    \centering
     \includegraphics[width=0.5\textwidth]{Figure_file/plane_wave_setup_202005.jpg}
    \caption{Schematic of the transmittance measurement setup. Additional details are given by Komatsu et al. (Ref.~\onlinecite{kkomatsu}).
    \label{fig:plane_wave_setup} }
\end{figure}

\begin{figure}
    \centering
%    \includegraphics[width = 0.5\textwidth]{Figure_file/flat_sample_losstan.jpg}
%    \includegraphics[width = 0.5\textwidth]{Figure_file/flat_sample_losstan_v02.png}
    \includegraphics[width = 0.5\textwidth]{Figure_file/Data_TransVsFreq_DiffVsFreq_FlatDisk.png}
        \caption{Top Panel: Transmittance measurement of the flat sample  (blue data) and two-parameter fit (solid orange) including the index of refraction and loss tangent. The measurement was done in five sub-bands indicated by horizontal bars. Bottom panel: residual, data minus fit, from which we infer error bars. We conservatively take the error bar per datum in each sub-band to be the RMS of the residual in the sub-band.
    \label{fig:flat_measurement} }
\end{figure}

We measured the transmittance of each sample and of both mechanically attached flat-side to flat-side.  The two samples were held together; no glue was used. The samples were stacked with $x$ orientations aligned parallel to each other. Each of the measurements was conducted with the transmission axis of the wire grid polarizers parallel and perpendicular to the $x$ axis of the samples. We refer to these measurements as $T_{x}$ and $T_{y}$, respectively, indicating that the incident and measured polarization states align with the $x$ and $y$ orientations of the samples. The measurements are shown in Figure~\ref{fig:pharos_trans} together with the predicted transmission, which was calculated using RCWA and was based on the average values given in Table~\ref{tab:geometrical_measurement_parameters_table} and no loss. The transmittances $T_{x}$ and $T_{y}$ of individual samples agree with predictions and are only $\sim$0.75 because they were patterned only on one side. 

\begin{figure*}[tbp]
    \centering
    \includegraphics[width=1.0\textwidth]{Figure_file/pharos89_measurement_20200529.jpg}
    \caption{ Transmittance measurements $T_{x}$ and $T_{y}$ (blue data) of each sample (top four panels), of the samples stacked flat side to flat side (bottom row), and transmission predictions (red lines) based on the measured mean parameters given in Table~\ref{tab:geometrical_measurement_parameters_table}. In the bottom row, the plates are stacked with $x$ of one parallel to $x$ of the other.
    %\comred{need to change labeling of Figures} 
    \label{fig:pharos_trans} }
\end{figure*}

For the stacked samples we find 91\% transmittance averaged between the $T_{x}$ and $T_{y}$ data for the lowest LiteBIRD frequency band between 34 and 46 GHz. For the second lowest band between 43 and 58 GHz the average is 97\%. Other frequency bands have above 98\% averaged transmittance. At frequencies above 150~GHz the transmittance of the stack is decreasing and is lower than predicted. A $\chi^{2}$ analysis using data over the entire bandwidth (33-190~GHz) and varying the loss tangent in the fit model gives a minimum for $\tan \delta < 1\cdot 10^{-4}$, which is consistent with measurements with the native sample. 

While determining the precise source for lower transmittance at higher frequencies is beyond the scope of this paper, we discuss several candidates. Calculations indicate that a uniform 30~$\mu$m air gap between the stacked samples could explain the observed feature. Measurements set an upper limit of 24~$\mu$m. Ruze scattering from a flat surface with 30~$\mu$m RMS roughness could decrease transmittance to 95\% at 180~GHz~\cite{1446714}. This roughness value is close to the 30~$\mu$m uncertainty we quote for SWS height measurements (see Table~\ref{tab:geometrical_measurement_parameters_table}), which could be interpreted as an effective roughness. However, transmission measurements of the single samples indicate lower levels of effective roughness. 
%\sout{Laser ablation of the SWS modifies the material properties near the surface and the modified material may exhibit higher loss compared to the native single crystal.}
Evidently, any such higher loss is not sufficiently prominent to be exhibited with significant signal-to-noise ratio with transmission measurements of the individual samples. 
A combination of these effects could be the source for the lower transmission. 

%\comcyan{We list up the potential causes: the air gap between the two stacked samples, the diffraction, the scattering, and finally the change of the material properties. First, we set the upper limit of the air gap between the stacked samples as $14\pm 10~\mu$m by taking the difference between the thickness of the stacked sample and the sum of the two individual samples. We computed the transmittance of the stacked sample including the uniform air gap. A minimum of 30~$\mu$m of the air gap is necessary in order to account the observed feature. The effect of the air gap should only appear when the two samples are stacked. Although we have the transmittance measurement of the two individual samples, it is not clear to conclude the presence of the feature at the individual sample measurements due to the residual systematic noise.
%%We measure the potential air gap between the samples and we set an upper limit of 24~$\mu$m. Therefore, a part of the cause may be due to the airgap effect. 
%The diffraction is the effect that tends to appear at the high frequency side. In our SWS design, onset of the diffraction is expected at 182~GHz. Furthermore, the general tread of its feature is a sharp drop in the transmittance, and thus the broad suppression of the transmittance cannot be explained by the diffraction effect. The effect of a scattering can suppress the transmittance at the higher frequency range. The surface with the SWS array is not a flat, and thus it is difficult to define a surface for the scattering. Nevertheless, we can imagine a hypothetical surface after removing the perfectly periodic SWS array from the sample. If this surface has any random surface error, we can estimate the loss of efficiency using Ruze's equation. The RMS random surface error is 20-30~$\mu$m can decrease the transmittance to 98-95\% at 180~GHz if the transmittance is 1 without any scattering. The current estimate of the SWS height has an error of 40~$\mu$m (Table~\ref{tab:geometrical_measurement_parameters_table}). This error includes the variation from the tip of the SWS and the variation of the bottom of the pyramidal shape, and thus we cannot deny the possibility that a part of the suppression in transmittance may come arise due to the scattering. The laser machining relies on the ablation by the high power laser interacting with a material. Any leftover region of the material after the machining may be altered its material properties. In order to support the data with this hypothesis, the material properties, the index of refraction and the loss-tangent, appear to be altered in frequency dependent manner. Thus the model and the data agree well below 150~GHz, and the difference appear above 150~GHz. We cannot deny this hypothesis and it requires a further investigation in the field of the material science. We listed these possibilities, and we leave the future report for further investigations. (**Please check.**)}
%While it is difficult to deny this possibility, we know that the model prediction agree to the data in general except this high frequency region. 
%While the magnitude of the suppression and the error of the height are comparable, it is difficult to conclude the cause definitively and we cannot exclude the possibility of the scattering. 
%The random surface error is difficult to define to the SWS, but the required RMS random surface error is in the order of the spot diameter of a laser, and thus there is no reason to exclude as a candidate. 
%TO BE COMPLETE by rerun the comparison for a single sample with the Ruze's equation. 
%Finally, a change in material properties is a possibility but there is not sufficiently prominent in the measurement of individual samples}
%It may arise from a small air gap between the stacked samples, increased scattering that %isn't sufficiently prominent in the measurement of the individual samples, or change in %material properties that is again not sufficiently prominent in the measurement of %individual samples. 
%\comblue{\sout{1. measuring stack thickness; 2. checking consistency of stack vs. individual measurement} } 

%\comgreen{$\chi ^2$ calculation shows that $\tan{\delta} = 2.44\times 10^{-4}$ is not the smallest $\chi ^2$ in $x$ and $y$ direction, But the difference is so small betwen no loss tangent and $\tan{\delta} = 2.44\times 10^{-4}$. Which number should I use? I made the figure in the slide, and I think I can use $\tan{\delta} = 2.44\times 10^{-4}$}


==> sec_conclusion.tex <==

SWS have advantages as ARC because they obviate the need for multiple materials and glues with precisely tuned indices of refraction, and because the index gradient produced can be smoother and tailored to specific applications. SWS are superior for cryogenic applications, because there is no need to match materials with different coefficients of thermal expansion.  Fabricating SWS on alumina and sapphire -- materials that have favorable optical properties in the millimeter and sub-millimeter wave band -- using standard machining approaches has been challenging because both materials are among the hardest available. They rank 9/10 on the relative hardness Mohs scale, and sapphire (alumina) has a value of 2500 (2000) HV on the Vickers hardness scale. In this paper we have extended our development of laser ablation as a tool to fabricate SWS for the millimeter and sub-millimeter band. We demonstrated structures on sapphire with aspect ratio $a = 3.7$. The newly fabricated SWS give a working bandwidth of 130\% with transmission above 90\% centered on 97~GHz, and of 116\% with transmission of at least 97\% centered on 102~GHz, arguably the largest bandwidths yet demonstrated in this wavelength range.

Using shorter pulse duration higher power laser and a more efficient fabrication process we have accelerated the AVRR for sapphire by a factor of 18 to 1.6 mm$^{3}$/min. Further acceleration is achievable with increase in laser power~\cite{Neuenschwander,boerner2019} and improvements in fabrication efficiency.

Although the native material was  non-birefringent we found shape asymmetries in the fabricated SWS. The origin of the asymmetries is yet to be understood. However, calculations show that proper relative alignment of samples reduces the magnitude of induced instrumental polarization due to differential reflection by a factor of 35 to 0.07\% at normal incidence, and to less than 0.6\% for incidence angles up to 20 degrees. Measurements at normal incidence are consistent with these predictions as they show the expected reduction in instrumental polarization, but are currently limited to an upper limit of 1\%.

These results and newer ones showing even higher ablation rates~\cite{wen_inprep} indicate that laser ablation of SWS on sapphire and on other hard materials such as alumina is an effective way to fabricate broad-band ARC; the technique has particularly strong advantages in the case of cryogenic applications. 

==> sec_design.tex <==

%\comblue{I think the material in the next two paragraphs is needed, although it could go to the introduction, if so preferred. }


LiteBIRD's LFT, one of three telescopes aboard the spacecraft~\cite{sugai}, will operate over a frequency range between 34 and 161~GHz. The focal plane will have about 1200 bolometric detectors tuned to nine broad-band, $\sim$25\% fractional bandwidth frequency bands.  A single HWP placed at the entrance aperture of the LFT will modulate the polarization of sky signals across the entire bandwidth. Thus, the goal is to demonstrate SWS ARC with 130\% fractional bandwidth centered on 97~GHz.

Klopfenstein (Ref.~\onlinecite{Klopfenstein}) derived a prescription for impedance matching between free space and a sample of index $n$. The prescription gives an optimal index of refraction profile and depends on a parameter $\Gamma_{m}$ that controls the trade-off between the lowest frequency of the passband and transmission ripple in-band~\cite{Grann}. All values of $\Gamma_{m}$ between 0.01 and 0.1 give average band transmission between 98\% and 99\%, and we chose $\Gamma_{m} =0.055$ as a fiducial value. With this value average transmission is near 99\%. There are several approaches to transforming the index profile to a physical shape but there is no single closed-form solution~\cite{Grann, Chen:95}. 
%We use an empirical approach
We employ an empirical design approach: we construct physical shapes and use effective medium theory (EMT)~\cite{EMT} and rigorous coupled-wave analysis (RCWA)~\cite{1457488,Moharam} to calculate the resulting index profile. We choose the physical shape that most closely reproduces the desired Klopfenstein index profile. RCWA calculations were carried out using DiffractMOD~\cite{diffractmod}.

%augmented by calculations using effective medium theory (EMT)~\cite{EMT} and rigorous coupled-wave analysis (RCWA)~\cite{1457488,Moharam}. RCWA calculations were carried out using DiffractMOD~\cite{diffractmod}.

We model the SWS as a grid of identical pyramids, see Figure~\ref{fig:Shape_parameters}.  We search for a pyramid shape that closely matches the Klopfenstein index profile by constructing a shape function that gives the width of the pyramid as a function of distance $z$ from the substrate material
\begin{equation}
    w(z) = w_0 + \left\{(p-b)-w_0\right\}\left\{1-(z/h)^{\alpha}\right\},
%    \label{width}
\label{eq:alpha}
\end{equation}
where the parameters are defined in Figure~\ref{fig:Shape_parameters}. 
A value of $\alpha=1$ gives linear slopes; smaller (larger) values give concave (convex) slopes. We considered several values for $\alpha$, but in all cases used $p = 0.54$~mm and $h=2.0$ mm, giving $a=3.7$. The pitch $p$ is set by requiring that at normal incidence the smallest value of the highest pass-band frequency be $\nu_{high} = c/p \, n_{s} = 180$~GHz. Thus $p=\lambda_{high}/n_{s}=0.54$~mm, where $n_{s} = 3.06$ is the index of c-cut sapphire. Smaller value of $p$ implies shorter $\lambda_{high}$, higher $\nu_{high}$, and thus larger bandwidth. In Section~\ref{sec:non_normal} we discuss non-normal incidence. Guidance for the minimum required $h$ is obtained by considering the lowest pass-band frequency and applying the standard criterion for maximum transmission with a single ARC layer that has a uniform index $n_{l}$. In that case $n_{l}=\sqrt{n_{s}}$, and the thickness of the layer should be $t=\lambda_{0}/4n_{l}$, where $\lambda_{0}$ is the vacuum wavelength. 
%\comred{Since a Klopfenstein taper degenerates to a usual quarter-wavelength design if the change of impedance along the height adiabatically approaches 0, the height driven by the quarter-wavelength design is adopted here as a convenient reference.} \comblue{(SH: I don't understand what this says.)} 
For the pyramids we found empirically that $h$ should satisfy $h \gtrsim \lambda_{0}/3n_{l} = 1.9$~mm, where $\lambda_0=8.8~$mm.
%\comgreen{\cite{kamizuka}}. \comblue{The addition of this reference is out of place. the sentence says that "*we* found empirically ...", and then we give a reference to someone else's publication... Also, why has this been added? I looked at the paper and I don't quite see the connection to this sentence. } 
We required $h \geqq 2.0$~mm.
%\comcyan{Correspondingly, the aspect ratio, height/pitch$\equiv a$, is $a\geqq3.7$.}
The choice of $w_0$ was determined iteratively by trying several values. We determined that $w_0=0.1$~mm is the largest value that would still give an effective index that matches the Klopfenstein profile. Larger values produce a mismatch of the indices near $n=1$. We assumed that the deep laser ablated grooves will give $b=0$ making $p=p'$ (see Figure~\ref{fig:Shape_parameters}).
%\comgreen{\cite{tomo_ISSTT}}. \comblue{1. See earlier comment regarding citation 27; 2. Even if the citation is included properly, does the ISST paper *prove* that $p=p'$?}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{Figure_file/parameter_settings.jpg}
    \caption{Geometrical parameters of pyramidal-shaped SWS. The shape of the pyramids (right panel) is controlled by a parameter $\alpha$ defined by Equation~\ref{eq:alpha}. Other parameters are the tip width $w_0$, the period $p$, the width at the bottom of the pyramid $p^\prime$, the groove width $b$, and the height $h$.
    \label{fig:Shape_parameters} }
\end{figure}
We used second-order EMT to calculate the effective index of refraction as a function of $\alpha$, and RCWA to calculate the expected transmission as a function of frequency; see Figure~\ref{fig:RCWA_profile_trans}. A convex pyramid shape with $\alpha = 1.5$ gives an index profile that closely matches the Klopfenstein profile with the fiducial $\Gamma_{m}$. The average band transmissions for $\alpha = 1.0, \, 1.5$ and 2 are 97.7\%, 98.4\%, and 98.3\%, respectively; see Figure~\ref{fig:RCWA_profile_trans}. 
The sharp reflection features apparent in the Figure above 180~GHz are due to the onset of diffraction.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{Figure_file/alpha_dependence_20200507_ver4.jpg}
    \caption{Top: EMT-calculated index profiles for four values of $\alpha$ (colored lines, Equation~\ref{eq:alpha}), and the Klopfenstein index profile with $\Gamma_{m} = 0.055$ (black). The other physical parameters used to calculate the index profiles are $h=2.0$ mm, $p = 0.54$~mm, $w_0=0.1$~mm, and $b=0$. Bottom: calculated transmittance as a function of frequency for SWS designs with the parameters given in the upper panel. Sharp reflection features above 180~GHz are due to the onset of diffraction. 
    \label{fig:RCWA_profile_trans} }
\end{figure}




==> sec_discussion.tex <==




%\sout{The two-dimensional rectangular-like nature of the $z$-axis projection of the SWS is a potential source of polarimetric systematic effects.}
Systematic asymmetry in fabrication along the two orthogonal axes, due to laser beam polarization or birefringent material properties (if such is used), leads to different effective indices of refraction along the two axes. Differential index causes differential transmission, which is a source of instrumental polarization (IP), the conversion of unpolarized to polarized light by the optical element. Even when the structures are two-dimensional symmetric there is differential reflection at non-normal incidence, as there would with any ARC scheme; differences in transmission between S and P polarization states of the incident light lead to IP. 

To quantify the IP induced by normal incidence differential transmission we use the figure of merit~\cite{radio_astronomy,karl} 
\begin{align}
    {\rm IP}(\nu) & =  \frac{ T_x(\nu) - T_y(\nu)  }{T_x(\nu) + T_y(\nu)} 
\label{eq:asymmetry_nophi} \\
    & =  \frac{ T(\phi=0^{\circ}, \nu) - T(\phi=90^{\circ}, \nu)  }{T(\phi=0^{\circ}, \nu) + T(\phi=90^{\circ}, \nu)} ,
\label{eq:asymmetry_phi1}
\end{align}
where we have introduced in the last expression the relative rotation angle $\phi$ between the $x$ orientation of the sample and the direction along which transmission is probed. IP vanishes for normal incidence light when the substrate and ARC are $z$-projected isotropic. At normal incidence  Equations~\ref{eq:asymmetry_nophi} and~\ref{eq:asymmetry_phi1} could have been written equivalently in terms of $T_{s} \equiv T(\phi=0^{o}) $ and $T_{p} \equiv T(\phi=90^{o})$, the transmissions for S and P polarization states.
 
At non-normal incidence and in the presence of $x$-$y$ ARC asymmetry $T_{s}$ and $T_{p}$ depend on both the angle of incidence $\theta_{i}$ and on the azimuthal angle $\phi$ of the plane of incidence, measured relative to $x$. We now have  
 \begin{equation}
    {\rm IP}(\phi,\theta_i,\nu) = \frac{ T_s(\phi,\theta_i,\nu) - T_p(\phi,\theta_i,\nu)  }{T_s(\phi,\theta_i,\nu) + T_p(\phi,\theta_i,\nu)}
\label{eq:asymmetry_phi2}
\end{equation} 
see Figure~\ref{fig:inc_pol_iamge}.
%\comblue{the equation uses $\theta_{i}$, the figure uses $\theta$. Please make uniform}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figure_file/pol_image.jpg}
    \caption{A diagram showing the variables of Equation~\ref{eq:asymmetry_phi2}. The transmissions $T_{p}$ and $T_{s}$ are for light polarized parallel and perpendicular to the plane of incidence, respectively.}
    \label{fig:inc_pol_iamge}
\end{figure}

In the following two Sections we quantify systematic effects due to asymmetry in the fabricated SWS at normal incidence (Section~\ref{sec:asymmetry}) and due to non-normal incidence (Section~\ref{sec:non_normal}), and discuss the level of mitigation provided by appropriately stacking the two-disc sandwich. We refer to `parallel' and `perpendicular' configurations, in which the two plates are stacked with their $x$ axes parallel, or with $x$ of one perpendicular to $x$ of the other, respectively. In the perpendicular configuration the quantities $T_{x}$ and $T_{y}$ refer to transmission measurements relative to the $x$ axis of the source-side sample of the stack, which was Sample1. 

\subsection{Asymmetry of SWS at normal incidence}
\label{sec:asymmetry}

Figure~\ref{fig:IP} shows IP inferred from the measured data (Figure~\ref{fig:pharos_trans}) for the individual samples and when stacked in the parallel and perpendicular configurations. It also shows the calculated response (using RCWA) using the average parameters for the $x$ and $y$ orientations in Table~\ref{tab:geometrical_measurement_parameters_table}. We find values of IP reaching 10\% at frequencies below 100~GHz for the individual samples, and below 50~GHz for the parallel stacking. For the entire bandwidth the RMS IP is 2.5\%. 
At frequencies higher than 50~GHz, 
IP in the parallel stacking configuration is smaller than in the individual samples because of higher transmission and because of some averaging of the two somewhat different asymmetries. 

However, when the plates are stacked in the perpendicular configuration we find lower IP across the band as shown in the bottom panel of Figure~\ref{fig:IP}. 
The data and the RCWA prediction are consistent within measurement errors, which take into account residual standing waves (see Section~\ref{sec:transmission}).
If the errors are assumed to be statistical, we find an upper limit of 1\% on the RMS across the band. 
The RMS IP calculated based on RCWA is 0.07\%, a value that is nearly 35 times smaller than in the parallel configuration, and is below our  measurement limits.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figure_file/20191107_pharos89_measurement_IP_v4.jpg}
    \caption{
    Instrumental polarization due to differential transmission IP for each of the samples and when stacked with $x$ axes parallel and perpendicular (blue data points), and RCWA predictions for IP (solid, red) based on the average measured values (Table~\ref{tab:geometrical_measurement_parameters_table}). For perpendicular stacking, calculated RMS IP for the bandwidth is 0.07\%. The vertical dashed line shows the 90~GHz frequency for which we made measurements as a function of stack rotation angle; see Figure~\ref{fig:rotation}.
    \label{fig:IP} }
\end{figure}{}

Figure \ref{fig:rotation} gives data and RCWA predictions for normal incidence transmittance as a function of stacked sample rotation angle $\phi$ for the two configurations at 90~GHz. Concentrating on the parallel configuration first, the effective differential index in $x$ and $y$ is an effective stack birefringence that causes 8.6\% modulation as a function of $\phi$ with $\pi/2$ periodicity only with fully polarized incident light. 
That is, the measurements, which were conducted with fully polarized light, give
 \begin{equation}
    0.086 = \frac{ \bar{T}(\phi=0^{\circ}) - \bar{T}(\phi=45^{\circ})  }{\bar{T}(\phi=0^{\circ}) + \bar{T}(\phi=45^{\circ})}, 
\label{eq:asymmetry_phi}
\end{equation} 
with $\theta_{i} = 0^{o}$, $\nu=90$~GHz, and $\bar{T}$ indicates that we average all $T$ values at the $\phi$ indicated and with $\pi/2$ periodicity. If the experiment and simulation were conducted with partially polarized or  unpolarized light, this $\pi/2$-periodic modulation would have diminished or vanished, respectively. For the HWP, SWS using a-cut sapphire, $\pi/2$ effect also could be vanished with unpolarized light. For Given measurement errors in this band of frequencies, the $\pi/2$-periodic modulation of 0.086 has an uncertainty of 0.014. 

The IP signal due to differential transmission has $\pi$ periodicity. Given the $1\sigma = 1.4\%$ measurement uncertainty the data only give a $2\sigma$ upper limit of IP $<2.8\%$, when calculated using Equation~\ref{eq:asymmetry_phi1}. 
This value is consistent with the IP value at 90~GHz in the third panel of Figure~\ref{fig:IP}, $3 \pm 1.4\%$. This level would persist if the measurement was done with unpolarized light. 
In the perpendicular configuration both the $\pi/2$ and $\pi$-periodic modulation amplitudes, calculated using Equations~\ref{eq:asymmetry_phi} and \ref{eq:asymmetry_phi1}, are consistent with zero within measurement errors. 

The transmission data as a function of $\phi$, such as presented in Figure~\ref{fig:rotation}, reveal that measurements at only two orientations $x \, (\phi=0)$ and $y\, (\phi=90^{o})$ as shown in Figure~\ref{fig:IP} and IP calculated using Equation~\ref{eq:asymmetry_nophi} combine information from distinct physical effects. The effects correspond to, and can be quantified with higher accuracy using decomposition to Fourier harmonics\cite{Hanany:05,kkomatsu}. We fit the data of Figure~\ref{fig:rotation} to the model  
\begin{align}
    &T(\phi,\nu=90\mbox{~GHz})  =  & \nonumber \\
    &    a_0 + a_2\cos{(2\phi + 2C_2)} + a_4\cos{(4\phi + 4C_4),} &
    \label{eq:fourier}
\end{align}
and constrain the amplitudes and phases. We find 
IP$=a_2/a_0=1.6 \pm 0.2\%$ and $0.21\pm 0.22\%$, in the parallel and perpendicular configurations, respectively; and $a_4/a_0 = 7.9\pm 0.2\%$ and $0.07\pm 0.22\%$, respectively, for the effect of stack birefringence. The data in the perpendicular configuration is consistent with zero we thus quote an upper limit of 0.5\% on the values of $a_2/a_0$ and $a_4/a_0$. 
We find that (1) 
the $\pi$ and $\pi/2$ periodic modulations quantified through $a_2/a_0$ and $a_4/a_0$ are more tightly constrained compared to using Equations~\ref{eq:asymmetry_phi1} and~\ref{eq:asymmetry_phi}; (2) the modulation amplitude constraints calculated using the two techniques are consistent; (3) there is a significant detection of IP, that is, $\pi$ periodic modulation, in the parallel case but not in the perpendicular case; and (4) the relatively large 7.9\% $\pi/2$ periodic modulation measured in the parallel case is not detectable in the perpendicular case. 

With the structures as fabricated, perpendicular stacking is predicted to constrain IP to below 0.5\% at 90~GHz, a value that is limited by measurement uncertainty, not by inherent asymmetry. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figure_file/pharos89_rotation_20200703.jpg}
    \caption{Stacked sample transmittance at 90~GHz (blue points) as a function of stack rotation angle $\phi$ for the parallel (top two panels) and perpendicular (bottom two panels) configurations, and RCWA predictions based on the measured parameters in Table~\ref{tab:geometrical_measurement_parameters_table} (red solid). The lower panel in each pair has a limited range for the ordinate values. Shaded regions indicate the 2\% systematic uncertainty we assign to each data point in this frequency. The statistical uncertainty per data point is 0.2\%.
    \label{fig:rotation} }
\end{figure}{}


\subsection{Non-normal incident light}
\label{sec:non_normal} 


Optical systems are designed to admit rays over a range of incidence planes and angles and thus  
calculations of systematic effects arising from ARC SWS asymmetry should take account of the entire range of incidence planes and angles. Including the full range amounts to averaging that gives smaller systematic effects compared to using a single incidence plane and the extreme incidence angle. In the discussion below we analyze the effects of non-normal incidence angles {\it without} any such averaging, and therefore the quantitative values should be understood as upper limits. The analysis relies solely on RCWA calculations of the perpendicular configuration; we have already established that this configuration has smaller level of systematic effects. 

The upper panel of Figure \ref{fig:pharos89_inc} shows calculated IP$(\phi=0)$ as a function of frequency for normal incidence and for the 5, 10, 15 and 20 degrees incidence angle.  For normal incidence the calculation is identical to the one shown in the lower panel in Figure~\ref{fig:IP}. The lower panel shows the difference between transmission at normal incidence and at other angles, again for $\phi=0$. For LiteBIRD's maximum planned incidence angle of 15 degrees RMS IP across the band is 0.4\%, an increase of 0.3\% relative to normal incidence. At 20~degrees incidence, RMS IP increases to 0.6\%. For $\phi=90$ degrees, RMS IP values at 15 and 20 degrees incidence are smaller by 0.1\%.  

Onset of diffraction is apparent at lower frequencies with larger incidence angles. For off-normal incidence, the frequency of diffraction onset -- that is, at the lowest order -- is~\cite{Grann,Bruckner:07}
\begin{equation}
    \nu_{d} = \frac{c}{p(n+\sin{\theta_i})},  
\label{eq:diffraction}
\end{equation}
providing qualitative agreement with the RCWA calculation. We do not expect exact quantitative agreement because the RCWA calculation assumes the full average shape information for the two samples, as given in Table~\ref{tab:geometrical_measurement_parameters_table}, whereas Equation~\ref{eq:diffraction} only assumes a periodic array of scattering centers. 


\begin{figure}[h]
    \centering
    \includegraphics[width = 0.48\textwidth]{Figure_file/pharos89_incident_20200612.jpg}
    \caption{RCWA prediction of IP$(\phi=0)$ for various incidence angles (upper panel), and the difference of off-normal incidence spectra with normal incidence spectra (lower panel), all in the case of perpendicular stacking configuration.
    \label{fig:pharos89_inc} }
\end{figure}{}





==> sec_fabrication.tex <==


\subsection{Sapphire}
\label{sec:sapphire}

%We procured three samples of c-cut sapphire
%\comred{, cut perpendicular to the c-axis,} from the same ingot
We procured three samples of c-cut sapphire that were cut from the same ingot, each $3.150 \pm 0.002$~mm thick and 100~mm diameter. 
%\comblue{If the referee doesn't know what c-cut is, why would he know what c-axis is? I think we should push back here. This is too trivial to include. A 3 sec google search would tell anyone what c-cut is.} 
We used one sample and the apparatus discussed in Section~\ref{sec:transmission} to measure the index of refraction and loss and obtained $n=3.062 \pm 0.002$ and $\tan{\delta}<1\times10^{-4}$, which is consistent with other data~\cite{Lamb}. In subsequent analysis and simulations we assume that these values are common to all three samples. 
%\comblue{Two topics in progress: 1. significant figures; 2. how to report loss.}

We fabricated the SWS on a circular area of 34.5~mm diameter on one side of each of two samples, to which we refer as Sample 1 and Sample 2. We patterned only one side because LiteBIRD's LFT HWP will be a Pancharatnam multi-stack achromatic HWP~\cite{Pancharatnam1} with SWS only on the outermost surfaces. 
In Section~\ref{sec:transmission} we present transmission measurements of each sample and when they are stacked flat side on flat side. 

Using c-cut, non-birefringent sapphire, simplifies interpretation of the results. At normal incidence, which is the only experimental data we present here, any apparent birefringence is the result of asymmetry in fabrication, not of inherent asymmetry in the material, as would be the case with birefringent a-cut sapphire.




%about laser machine, scan strategy
\subsection{Laser machining}
\label{sec:laser}

The SWS are patterned using a 15~W average power femto-second laser operating at 1030~nm; the laser parameters are given in Table~\ref{tab:laser_specification}. 
The laser beam scans lines in two orthogonal directions to make grooves, and thus produce the pyramids; see Figure~\ref{fig:scan_strategy}. This scan strategy largely follows an approach we used in the past, see for example Young et al. (Ref~\onlinecite{karl}).
The focus position is set at a fixed $z=-0.75$~mm throughout the ablation. The surface of the disk at the beginning of ablation is at $z=0$ and negative values are inside the sample.

\begin{table}[h]
    \centering
    \caption{Laser Specifications}
    \begin{tabular}{c|c}\hline
        \multicolumn{2}{c}{Model:  Pharos, PH1-15W} \\ \hline
         Wavelength & 1030 nm \\
         Repetition rate &  75 kHz\\
         Pulse duration & 290 fs \\
         Pulse energy & 200 $\mu$J \\ %\hline
%\multicolumn{2}{c}{Galvano scanner with f-theta lens (ScanLab)}\\\hline
%         focus distance & 100 mm\\
         Spot diameter ($1/e^2$) & 15.5 $\mu$m \\
    \end{tabular}
    \label{tab:laser_specification} 
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width = 0.4\textwidth]{Figure_file/scan_strategy_20200522.jpg}
    \caption{Sketch of the laser beam scan pattern to fabricate the SWS. Repeated ablation of groups of 53 lines produces grooves. The lines are internally spaced by less than 10 $\mu$m and the groups are separated by at least 72~$\mu$m.  Grooves fabricated in two orthogonal directions leave pyramids, which are the SWS. Layers similar to the one shown in the sketch are repeated 60 times until the desired SWS height is achieved. } 
    \label{fig:scan_strategy}
\end{figure}


\subsection{Characterization of fabricated structures}
\label{sec:charaterization}

The SWS were imaged using confocal imaging. A three-dimensional image of a section of the fabricated region is shown in Figure~\ref{fig:sample_shape}.   Visual inspection indicates that all SWS are physically intact with no breakage nor damaged tips. We measured 160 structures at each of five  locations in each sample, in the center and in four edge regions, and quantified several geometrical parameters as detailed in Figure~\ref{fig:sample_shape} and Table~\ref{tab:geometrical_measurement_parameters_table}. Values given in the Table are averages and standard deviations of the 800 measurements. We established a global cartesian coordinate system that was aligned with the grooves, and for each measured pyramid we defined $xz$ and $yz$ planes that intersected the center of its peak. For both planes (and for each pyramid) we quantified the widths $w_{0x}$ and $w_{0y}$ and two `saddle' heights $d_{x}$ and $d_{y}$, which quantified the depths between pyramids in the $x$ and $y$ directions. The total height $h_{t}$ is given by the depth into trenches in the diagonal direction where the laser beam ablates in both the $x$ and $y$ passes. We best-fit the slopes of the pyramids as imprinted in the $xz$ and $yz$ planes to produce measured $\alpha_{x}$ and $\alpha_{y}$.

\begin{figure}[t]
    \centering
%    \includegraphics[width=0.5\textwidth]{Figure_file/pharos89_shape_ver20200420.jpg}
%    \includegraphics[width=0.5\textwidth]{Figure_file/pharos89_shape_20200512.jpg}
    \includegraphics[width=0.5\textwidth]{Figure_file/pharos89_shape_20200518.jpg}
    \caption{  Left: Confocal microscopy image of a section of the fabricated SWS. The structures are physically intact across the entire sample and the average height is 2~mm. Right: Definition of measurement parameters. Averages of 800 measurements of these parameters are given in Table~\ref{tab:geometrical_measurement_parameters_table}.   
    \label{fig:sample_shape} }
\end{figure}


There is good agreement between the design and fabricated values for the pitch and total height, and there is $x$-$y$ symmetry in the measured pitch. There is good repeatability between the two samples, which were fabricated several days apart. Asymmetry of 5\%-20\% is apparent at the tip of the structures, the saddle heights, and the slope values $\alpha$. This structural asymmetry could have been caused by laser beam polarization, which was not monitored; by the ablation scan strategy, for example the order in which $x$ and $y$ directions were scanned; or by laser beam projection, if the sample was not precisely normal to the beam.
%We will discuss the systematic effects caused by the structure asymmetry in the later section.

It took 10.5~hours to fabricate each sample giving an average volume removal rate (AVRR) of 1.6~mm$^{3}$/min. This rate is 18 times faster than achieved in one of our earlier publications~\cite{tomo_ISSTT}. The higher rate is due to using five times higher averaged power and a more efficient sample scan pattern. Matsumura et al.\ (Ref.~\onlinecite{tomo}) report a higher AVRR of 2.2~mm$^3$/min, but with higher power (25~W) and for SWS with smaller total height of 715~$\mu$m; Schuetz et al.\ (Ref.~\onlinecite{victor}) show that AVRR increases with power and lower structure height. 


Using EMT and the average values given in Table~\ref{tab:geometrical_measurement_parameters_table} we calculated effective index profiles in $x$ and $y$ for each sample; see Figure~\ref{fig:pharos8_9_EMT}. To indicate the variance we included the index profiles for all 800 measured structures as shaded regions. As the values in Table~\ref{tab:geometrical_measurement_parameters_table} indicate, the measured profiles in $x$ match the design profile with $\alpha = 1.5$ better than the measured profiles in $y$.

\begin{table}[t]
    \centering
    \caption{
    Averages of measured geometrical parameters of 800 pyramids measured in five regions of each sample. The parameters are defined in Figure~\ref{fig:sample_shape}. The accuracy of the confocal microscope is 1~$\mu$m in the $xy$ plane and 8~$\mu$m in the $z$ direction.}
    \begin{tabular}{c|c|c|c}
         Parameter     &    Design value & Sample 1 & Sample 2  \\ 
                       &    (mm) & (mm)      & (mm) \\ \hline
        Top width $x$ ($w_{0x}$) & 0.1 & $0.14 \pm 0.01 $ & $0.14 \pm 0.01 $\\
        Top width $y$ ($w_{0y}$) & 0.1 & $0.12 \pm 0.01 $ & $0.12 \pm 0.01 $\\
        Saddle height $x$ ($d_{x}$) & & $1.51 \pm 0.04 $ & $1.52 \pm 0.04 $\\
        Saddle height $y$ ($d_{y}$) & & $1.60 \pm 0.04 $ & $1.59 \pm 0.05 $\\
        Total height ($h_{t}$) & 2.0 & $2.03 \pm 0.04 $ & $2.04 \pm 0.05 $\\
        Pitch $x$ ($p'_{x}$) & 0.54 &  $0.54 \pm 0.01 $ & $0.54 \pm 0.01 $\\
        Pitch $y$ ($p'_{y}$) & 0.54 & $0.54 \pm 0.01 $ & $0.54 \pm 0.01 $\\ \hline 
        $\alpha_x$ $^{\dagger}$ & 1.5& $1.56 \pm 0.06 $ & $1.56 \pm 0.04$\\
        $\alpha_y$ $^{\dagger}$ & 1.5 & $1.22 \pm 0.02 $ & $1.22 \pm 0.02$\\
\hline
\multicolumn{3}{l}{$^{\dagger}$ dimensionless quantity}
    \end{tabular}
    \label{tab:geometrical_measurement_parameters_table}
\end{table}

\begin{figure}[h]
    \centering
%    \includegraphics[width=0.45\textwidth]{Figure_file/pharos89_effn.jpg}
    \includegraphics[width = 0.5\textwidth]{Figure_file/pharos89_effective_index_20200608.jpg}
    \caption{ The effective index of refraction calculated with EMT using the average values of the measured SWS (solid red and green), and with the design values and $\alpha = 1.5$ (solid black). The shaded regions include index profiles for all 800 measured structures.
    \label{fig:pharos8_9_EMT} }
\end{figure}



==> sec_intro.tex <==


% 
Sapphire, alumina, and silicon have material properties that make them appealing for use as optical elements in the millimeter and sub-millimeter (MSM) waveband, loosely defined as 30 - 3000 GHz. Compared to plastic-based materials, they have indices of refraction near 3, giving more aberration correction power per unit lens thickness~\cite{Lamb}. They have amongst the lowest absorption loss at room temperature and when cooled to cryogenic temperatures \cite{parshin1995}, and they have thermal conductance higher by factors of hundreds, making them useful for cryogenic applications~\cite{child_1973}. Sapphire has 10\% birefringence making it an ideal half-wave plate (HWP) material for polarimetric applications. 
A number of astrophysical instruments operating in the MSM waveband are using these materials~\cite{Thornton_2016,EBEX2018,SPT-3G,Kaneko2020}. 

The high index of refraction leads to high reflection loss; the average reflectance across 30\% fractional bandwidth of a 1~cm thick slab of non-birefringent sapphire at 150~GHz is 40\%. Reduction of reflection loss is achieved by applying an anti-reflection coating (ARC).  There are two generic approaches for implementing ARC:
%
(i) applying layers of materials with appropriately chosen intermediate indices; and (ii) machining sub-wavelength structures (SWS) on the native optical element material~\cite{Raut2011AntireflectiveCA}. 
%\comblue{(Did you check what are 'resonant structures' in relation to ARC? I don't believe they are related to multi-layer ARC. `Adiabatic tapering' is used, but less often then SWS. I don't think we should use 'metamaterial'. I have no idea what it means; I don't think a definition exists. In summary: what we had was fine. It captures the basic physics.)}
%
%(i) \comred{resonant structures} applying layers of materials with appropriately chosen intermediate indices; and (ii) \comred{adiabatic structures, called as a metamaterial,} machining sub-wavelength structures (SWS) on the native optical element material~\cite{Raut2011AntireflectiveCA}. 
%
An advantage of the SWS approach is that it does not require new materials and glues. This advantage matches well the needs of cryogenic instruments in which differences in coefficients of thermal expansion make the application of multi-layers challenging. Another advantage is that SWS give flexibility in synthesizing any index profile between free space and the substrate material.
%\comred{A single layer coating equivalent ARC using SWS can be realized by an array of the periodic pillar structure or an array of holes. For a broader frequency coverage, prescriptions exist for index profiles that give fractional bandwidths exceeding 100\% with maximal, in some sense optimal, in-band transmission~\cite{Klopfenstein}. 
%This can be realized by fabricating the adiabatic structures.}
Prescriptions exist for index profiles that give fractional bandwidths exceeding 100\% with maximal, in some sense optimal, in-band transmission~\cite{Klopfenstein}. 

Two classes of MSM instruments that require broad-bandwidths and cryogenic optical elements are those mapping the spatial polarization of the cosmic microwave background radiation (CMB)\cite{Johnson_2007,EBEX2018,SPT-3G,Simon2018,Kaneko2020,SO-OverviewGalitzki10.1117/12.2312985,cmb-s4techbookfirsted}, and others measuring the properties of Galactic dust \cite{Dober_blastpol10.1117/12.2054419,blasttngLourie10.1117/12.2314396,nika2pisano2020}. A number of these instruments have used, or plan to use, sapphire as HWP polarization modulator. 
To reduce detector noise the HWP is maintained at cryogenic temperatures, typically near 4~K, and to increase instrument throughput a single HWP operates over a broad range of frequencies, making a single quarter-wave layer of ARC inadequate. Examples of relevant past instruments include Blastpol and EBEX, which had sapphire HWPs with operating bandwidth of 69\% and 109\%, respectively\cite{Dober_blastpol10.1117/12.2054419,EBEX2018}. The bandwidth of the EBEX HWP is the largest reported to date. Ongoing and future experiments include POLARBEAR2, Simons Observatory and LiteBIRD\cite{Kaneko2020,SO-OverviewGalitzki10.1117/12.2312985,sugai}. 

LiteBIRD is a Japanese-led space mission scheduled to be launched late in the next decade~\cite{sugai,YSakurai}. LiteBIRD's low frequency telescope (LFT), designed to operate between 34 and 161~GHz (a fractional bandwidth of 130\%), will have an aperture diameter of 40~cm with a HWP operating at 20~K. Currently no ARC technology on sapphire is available over this broad bandwidth. Implementing SWS ARC for the LiteBIRD HWP has motivated the developments we report in this paper.

Although SWS have advantages as ARC, their implementation on hard materials such as sapphire and alumina present fabrication challenges~\cite{Araujo2016,JAIN20021269,TUERSLEY1994377,machining_difficult}. Broad bandwidths require SWS with aspect ratios $a$ -- defined as height/pitch -- reaching four. 
Diameters of anticipated sapphire and alumina optical elements, which are reaching 80~cm\cite{AliCPTHong10.1093/nsr/nwy019}, require commercially viable machining speed.  
To overcome these challenges we demonstrated a technique to fabricate mm-wave SWS on sapphire, alumina, and silicon using laser micro-fabrication~\cite{tomo,karl,victor,tomo_ISSTT}.  
With laser ablation, which has already been used in the past to ablate these and other materials~\cite{Bonse2002,Ihlemann1995,WANG2004221}, there is no wear and tear of the machining tool. 
Even for materials that can be machined using conventional tools, laser ablation gives finer control of structure shapes, because laser spot diameters can be focused to smaller sizes than other tools. A spot diameter of 16~$\mu$m has been demonstrated at the IR~\cite{HSakurai}; smaller spot diameters are achievable in the UV.
%\comred{The size of the structure by laser machining is limited by the laser spot size, the order of ten micrometer corresponding to THz scale, and the example demonstrations have  been  explored~\cite{HSakurai}. An approach smaller than tens-of-micrometer scale is also developed at typically optical wavelength using a lithography technique, which has a limited applicability to larger structural size, about THz range.}
%\comblue{(SH Comment: I don't think what was written in red was correct. The paper cites 16 micron beam at 1028 nm. (1) this is not `tens-of-micrometer'; (2) at UV we should be able to go down to $\sim \times$10 smaller spot size, certainly less than `tens-of-micrometer'.) } 
Finer control of SWS shapes would give higher transmission over broader bandwidth.
%\comred{Furthermore, a smaller beam spot diameter, a few micrometers using UV laser, can potentially pushes the limit using SWS technology toward the shorter wavelength,}.

Sch\"{u}tz et al.\ and Matsumura et al.\ (Refs.~\onlinecite{victor,tomo}) demonstrated laser-ablated aspect ratios $a =$ 
%\comred{h/p =} 
2.2 and 2.5
%, \comred{where $h$ is the height and $p$ is the pitch},
and heights between 700 and 800~$\mu$m, with sapphire and alumina, respectively. 
%\comblue{(`aspect ratio' is defined above. The referee simply missed it. I added the symbol $a$ above. )}
Young et al.\ (Ref.~\onlinecite{karl}) extended the technique to silicon, showing $a=4$ with height near 700~$\mu$m. To demonstrate applicability to lower frequencies and broader bandwidths, Matsumura et al.\ (Ref.~\onlinecite{tomo_ISSTT}) fabricated structures with $a=5.3$ and total height of 2.1~mm on sapphire. In all of these cases, the volume ablation rate was small, making fabrication of large samples prohibitively expensive; for example, at the rate Matsumura et al.\ (Ref.~\onlinecite{tomo_ISSTT}) quoted for the 2.1~mm tall structures on sapphire it would have taken two months to fabricate a 10~cm diameter sample. 
Further steps in the development of laser micro-fabrication of mm-wave SWS include demonstrating ablation rates that would make commercial fabrication viable with SWS aspect ratios suitable for broad bandwidth applications~\cite{wen_inprep}. In this paper we present progress in the design, fabrication, and characterization of laser-ablated SWS ARC, aiming for 130\% fractional bandwidth ARC centered on 97~GHz with improved fabrication speed. 
In Section~\ref{sec:design}, we present the design of the SWS. Sections~\ref{sec:sample} and~\ref{sec:transmission} give details of the fabrication of two sapphire samples and their transmission properties. We discuss the results and give conclusions in Sections~\ref{sec:discussion} and~\ref{sec:conclusion}.




==> sec_measurement.tex <==



We measured the transmittance of the samples at normal incidence between 33 and 190~GHz. The apparatus, a schematic of which is shown in Figure~\ref{fig:plane_wave_setup}, consisted of a source of microwaves, an optical chopper operating at 30 Hz, two parabolic mirrors, a diode detector, and a lock-in amplifier. Between the two mirrors there was an aperture of 30 mm diameter, a sample holder, attenuators to reduce standing waves, and two always identically aligned wire grid polarizers with calculated efficiency exceeding 99\% across the bandwidth. The transmission axis of the polarizers was aligned to within 3~degrees with the $x$ axis of the samples, and the stacked samples were aligned relative to each other to within 0.5 degrees.

To further reduce the effects of standing waves our reported transmittance at each frequency is the average of two transmission measurements taken with the detector positioned at two locations spaced by $\lambda /4$ along the light path. Each transmission measurement is the ratio of power detected with the sample to the power detected without it. 

Measurements of transmission through one of the native samples establish error estimates for subsequent data analysis. We measured transmission using different RF sources at five sub-bands between 33 and 190~GHz; see the top panel of Figure~\ref{fig:flat_measurement}. 
%\comred{The statistical error bars in the transmission measurement are small and not visible in the Figure.} \comblue{check} \comcyan{Yes, it is a high SNR measurement and so the error bar is there ubt it's invisible in this plot.} 
We fit the transmittance to a model with two free parameters, the index of refraction and loss tangent, and find the residuals; see the bottom panel of Figure~\ref{fig:flat_measurement}.  We identify systematic residuals as arising from incomplete cancellation of standing waves and 
%\comred{for all subsequent analyses} \comcyan{this statement looks fine}
quote the RMS of the residual as the error of transmission measurements in each sub-band. They are 6\% (33-50~GHz), 3\% (50-75~GHz), and 2\% (75-190~GHz). 

The errors quoted in Section~\ref{sec:sapphire} for the values of the index of refraction and loss were derived by fitting the transmittance data using statistical errors with magnitude per band as given above and including uncertainty on the measurement of sample thickness. The index and loss errors are dominated by the thickness measurement uncertainty.

\begin{figure}[h]
    \centering
     \includegraphics[width=0.5\textwidth]{Figure_file/plane_wave_setup_202005.jpg}
    \caption{Schematic of the transmittance measurement setup. Additional details are given by Komatsu et al. (Ref.~\onlinecite{kkomatsu}).
    \label{fig:plane_wave_setup} }
\end{figure}

\begin{figure}
    \centering
%    \includegraphics[width = 0.5\textwidth]{Figure_file/flat_sample_losstan.jpg}
%    \includegraphics[width = 0.5\textwidth]{Figure_file/flat_sample_losstan_v02.png}
    \includegraphics[width = 0.5\textwidth]{Figure_file/Data_TransVsFreq_DiffVsFreq_FlatDisk.png}
        \caption{Top Panel: Transmittance measurement of the flat sample  (blue data) and two-parameter fit (solid orange) including the index of refraction and loss tangent. The measurement was done in five sub-bands indicated by horizontal bars. Bottom panel: residual, data minus fit, from which we infer error bars. We conservatively take the error bar per datum in each sub-band to be the RMS of the residual in the sub-band.
    \label{fig:flat_measurement} }
\end{figure}

We measured the transmittance of each sample and of both mechanically attached flat-side to flat-side.  The two samples were held together; no glue was used. The samples were stacked with $x$ orientations aligned parallel to each other. Each of the measurements was conducted with the transmission axis of the wire grid polarizers parallel and perpendicular to the $x$ axis of the samples. We refer to these measurements as $T_{x}$ and $T_{y}$, respectively, indicating that the incident and measured polarization states align with the $x$ and $y$ orientations of the samples. The measurements are shown in Figure~\ref{fig:pharos_trans} together with the predicted transmission, which was calculated using RCWA and was based on the average values given in Table~\ref{tab:geometrical_measurement_parameters_table} and no loss. The transmittances $T_{x}$ and $T_{y}$ of individual samples agree with predictions and are only $\sim$0.75 because they were patterned only on one side. 

\begin{figure*}[tbp]
    \centering
    \includegraphics[width=1.0\textwidth]{Figure_file/pharos89_measurement_20200529.jpg}
    \caption{ Transmittance measurements $T_{x}$ and $T_{y}$ (blue data) of each sample (top four panels), of the samples stacked flat side to flat side (bottom row), and transmission predictions (red lines) based on the measured mean parameters given in Table~\ref{tab:geometrical_measurement_parameters_table}. In the bottom row, the plates are stacked with $x$ of one parallel to $x$ of the other.
    %\comred{need to change labeling of Figures} 
    \label{fig:pharos_trans} }
\end{figure*}

For the stacked samples we find 91\% transmittance averaged between the $T_{x}$ and $T_{y}$ data for the lowest LiteBIRD frequency band between 34 and 46 GHz. For the second lowest band between 43 and 58 GHz the average is 97\%. Other frequency bands have above 98\% averaged transmittance. At frequencies above 150~GHz the transmittance of the stack is decreasing and is lower than predicted. A $\chi^{2}$ analysis using data over the entire bandwidth (33-190~GHz) and varying the loss tangent in the fit model gives a minimum for $\tan \delta < 1\cdot 10^{-4}$, which is consistent with measurements with the native sample. 

While determining the precise source for lower transmittance at higher frequencies is beyond the scope of this paper, we discuss several candidates. Calculations indicate that a uniform 30~$\mu$m air gap between the stacked samples could explain the observed feature. Measurements set an upper limit of 24~$\mu$m. Ruze scattering from a flat surface with 30~$\mu$m RMS roughness could decrease transmittance to 95\% at 180~GHz~\cite{1446714}. This roughness value is close to the 30~$\mu$m uncertainty we quote for SWS height measurements (see Table~\ref{tab:geometrical_measurement_parameters_table}), which could be interpreted as an effective roughness. However, transmission measurements of the single samples indicate lower levels of effective roughness. 
%\sout{Laser ablation of the SWS modifies the material properties near the surface and the modified material may exhibit higher loss compared to the native single crystal.}
Evidently, any such higher loss is not sufficiently prominent to be exhibited with significant signal-to-noise ratio with transmission measurements of the individual samples. 
A combination of these effects could be the source for the lower transmission. 

%\comcyan{We list up the potential causes: the air gap between the two stacked samples, the diffraction, the scattering, and finally the change of the material properties. First, we set the upper limit of the air gap between the stacked samples as $14\pm 10~\mu$m by taking the difference between the thickness of the stacked sample and the sum of the two individual samples. We computed the transmittance of the stacked sample including the uniform air gap. A minimum of 30~$\mu$m of the air gap is necessary in order to account the observed feature. The effect of the air gap should only appear when the two samples are stacked. Although we have the transmittance measurement of the two individual samples, it is not clear to conclude the presence of the feature at the individual sample measurements due to the residual systematic noise.
%%We measure the potential air gap between the samples and we set an upper limit of 24~$\mu$m. Therefore, a part of the cause may be due to the airgap effect. 
%The diffraction is the effect that tends to appear at the high frequency side. In our SWS design, onset of the diffraction is expected at 182~GHz. Furthermore, the general tread of its feature is a sharp drop in the transmittance, and thus the broad suppression of the transmittance cannot be explained by the diffraction effect. The effect of a scattering can suppress the transmittance at the higher frequency range. The surface with the SWS array is not a flat, and thus it is difficult to define a surface for the scattering. Nevertheless, we can imagine a hypothetical surface after removing the perfectly periodic SWS array from the sample. If this surface has any random surface error, we can estimate the loss of efficiency using Ruze's equation. The RMS random surface error is 20-30~$\mu$m can decrease the transmittance to 98-95\% at 180~GHz if the transmittance is 1 without any scattering. The current estimate of the SWS height has an error of 40~$\mu$m (Table~\ref{tab:geometrical_measurement_parameters_table}). This error includes the variation from the tip of the SWS and the variation of the bottom of the pyramidal shape, and thus we cannot deny the possibility that a part of the suppression in transmittance may come arise due to the scattering. The laser machining relies on the ablation by the high power laser interacting with a material. Any leftover region of the material after the machining may be altered its material properties. In order to support the data with this hypothesis, the material properties, the index of refraction and the loss-tangent, appear to be altered in frequency dependent manner. Thus the model and the data agree well below 150~GHz, and the difference appear above 150~GHz. We cannot deny this hypothesis and it requires a further investigation in the field of the material science. We listed these possibilities, and we leave the future report for further investigations. (**Please check.**)}
%While it is difficult to deny this possibility, we know that the model prediction agree to the data in general except this high frequency region. 
%While the magnitude of the suppression and the error of the height are comparable, it is difficult to conclude the cause definitively and we cannot exclude the possibility of the scattering. 
%The random surface error is difficult to define to the SWS, but the required RMS random surface error is in the order of the spot diameter of a laser, and thus there is no reason to exclude as a candidate. 
%TO BE COMPLETE by rerun the comparison for a single sample with the Ruze's equation. 
%Finally, a change in material properties is a possibility but there is not sufficiently prominent in the measurement of individual samples}
%It may arise from a small air gap between the stacked samples, increased scattering that %isn't sufficiently prominent in the measurement of the individual samples, or change in %material properties that is again not sufficiently prominent in the measurement of %individual samples. 
%\comblue{\sout{1. measuring stack thickness; 2. checking consistency of stack vs. individual measurement} } 

%\comgreen{$\chi ^2$ calculation shows that $\tan{\delta} = 2.44\times 10^{-4}$ is not the smallest $\chi ^2$ in $x$ and $y$ direction, But the difference is so small betwen no loss tangent and $\tan{\delta} = 2.44\times 10^{-4}$. Which number should I use? I made the figure in the slide, and I think I can use $\tan{\delta} = 2.44\times 10^{-4}$}

